Sample Size Planning for Classification Models

In biospectroscopy, suitably annotated and statistically independent samples (e. g. patients, batches, etc.) for classifier training and testing are scarce and costly. Learning curves show the model performance as function of the training sample size and can help to determine the sample size needed to train good classifiers. However, building a good model is actually not enough: the performance must also be proven. We discuss learning curves for typical small sample size situations with 5 - 25 independent samples per class. Although the classification models achieve acceptable performance, the learning curve can be completely masked by the random testing uncertainty due to the equally limited test sample size. In consequence, we determine test sample sizes necessary to achieve reasonable precision in the validation and find that 75 - 100 samples will usually be needed to test a good but not perfect classifier. Such a data set will then allow refined sample size planning on the basis of the achieved performance. We also demonstrate how to calculate necessary sample sizes in order to show the superiority of one classifier over another: this often requires hundreds of statistically independent test samples or is even theoretically impossible. We demonstrate our findings with a data set of ca. 2550 Raman spectra of single cells (five classes: erythrocytes, leukocytes and three tumour cell lines BT-20, MCF-7 and OCI-AML3) as well as by an extensive simulation that allows precise determination of the actual performance of the models in question.

==> fig-confmat.tex <==
% Confusion matrix, sensitivity, specificity & Co.
%
% (C) 2008 - 2012 C. Beleites 

\newcommand{\zufrac}[5]{
  \small
  \matrix at (#1) (#2-zaehler) [matrix of nodes, cells = {draw}, 
  nodes = {draw, text width = 1ex, text height = 0.75ex, text depth = 0.25ex},
  execute at empty cell = {\node{};},
  row sep = -0.5pt,
  column sep = -0.5pt,
  ampersand replacement=\&,
  #3
]{#4};
\draw[very thick] ([below = 0.5ex] #2-zaehler.south west) ++(-.5ex, 0pt) node[coordinate] (#2-west) {}  -- 
                  ([below = 0.5ex] #2-zaehler.south east) -- ++(+.5ex, 0pt) node[coordinate] (#2-east) {};

 \matrix (#2-nenner) at (#2-zaehler.south)  [below = 1ex, matrix of nodes, cells = {draw}, 
  nodes = {draw, text width = 1ex, text height = 0.75ex, text depth = 0.25ex},
  execute at empty cell = {\node{};},
  row sep = -0.5pt,
  column sep = -0.5pt,
  ampersand replacement=\&
]{#5};
}
\newcommand{\tdiag}[1][0.75em]{\tikz[x=#1, y=#1, tight background]{
    \draw [ultra thin] (0, 0) rectangle (1, 1);  
    \draw (0, 0) -- (1, 1);
  }%
}
\newcommand{\tmdiag}[1][0.75em]{\tikz[x=#1, y=#1, tight background]{
    \draw [ultra thin] (0, 0) rectangle (1, 1);  
    \draw (0, 1) -- (1, 0);
  }%
}

\newcommand{\thv}[1][0.75em]{\tikz[x=#1, y=#1, tight background]{
    \draw [ultra thin] (0, 0) rectangle (1, 1);  
    \draw (0, .5) --++ (1, 0);
    \draw (.5, 0) --++ (0, 1);
  }%
}
\newcommand{\tp}[1][0.75em]{\tikz[x=#1, y=#1, tight background]{
    \draw [ultra thin] (0, 0) rectangle (1, 1);  
    \fill (0.5, .5) circle (#1/25);
  }%
}

\usetikzlibrary{backgrounds} 

\tikzstyle{thin}+=[line width=0.5pt]
\tikzstyle{shade}=[fill = gray]
\tikzstyle{eqmat}=[matrix of math nodes, below, 
  ampersand replacement=\&, column sep = 0pt,
  nodes = {anchor = base west, fill =yellow}]
 \begin{figure}
% \centering
\subfloat[\label{fig:Z} confusion matrix]{%
\begin{scriptsize}
\begin{tikzpicture}[tight background]
  \matrix (cm) [matrix of nodes, %cells = {draw}, 
  nodes = {text width = 1.5ex, text height = 1ex, text depth = 0.5ex, anchor = base east},
  execute at empty cell = {\node[draw]{};},
  row sep = -0.5pt,
  column sep = -0.5pt,
  ampersand replacement=\&,
  ]{
    ~ \& A \& B \& C \\
    A \&   \&   \&   \\
    B \&   \&   \&   \\
    C \&   \&   \&   \\
  };
  \node at (cm-1-3.north) [above, text width = 12ex, text badly centered] {prediction};
  \node at (cm-3-1.west) [xshift = -1.5ex, text width = 12ex, text badly centered, rotate = 90] 
  {reference} ;
\end{tikzpicture}
\end{scriptsize}}
\subfloat[\label{fig:sens}  $\Sens_A$]{
  \begin{tikzpicture}
    \zufrac{0,0}{senscl}{}
    {
      |[shade]| \&           \&            \\
                \&           \&            \\
                \&           \&            \\
    }{
      |[shade]| \& |[shade]| \& |[shade]|  \\
                \&           \&            \\
                \&           \&            \\
    }
 \end{tikzpicture}
}
\subfloat[\label{fig:spez} $\Spez_A$]{
  \begin{tikzpicture}
    \zufrac{0,0}{senscl}{}
    {
                \&           \&            \\
                \& |[shade]| \& |[shade]|  \\
                \& |[shade]| \& |[shade]|  \\
    }{
                \&           \&            \\
      |[shade]| \& |[shade]| \& |[shade]|  \\
      |[shade]| \& |[shade]| \& |[shade]|  \\
    }
   \end{tikzpicture}
}
\subfloat[\label{fig:ppv} $\PPV_A$]{
  \begin{tikzpicture}
    \zufrac{0,0}{senscl}{}
    {
      |[shade]| \&           \&            \\
                \&           \&            \\
                \&           \&            \\
    }{
      |[shade]| \&           \&            \\
      |[shade]| \&           \&            \\
      |[shade]| \&           \&            \\
    }
 \end{tikzpicture}
}
\subfloat[\label{fig:npv} $\NPV_A$]{
  \begin{tikzpicture}
    \zufrac{0,0}{senscl}{}
    {
                \&           \&            \\
                \& |[shade]| \& |[shade]|  \\
                \& |[shade]| \& |[shade]|  \\
    }{
                \& |[shade]| \& |[shade]|  \\
                \& |[shade]| \& |[shade]|  \\
                \& |[shade]| \& |[shade]|  \\
    }
   \end{tikzpicture}
}
\caption{ Confusion matrix \protect\subref{fig:Z} and characteristic fractions
  \protect\subref{fig:sens} -- \protect\subref{fig:npv}. The parts of the confusion matrix summed as
  enumerator and denominator for the respective fraction with respect to class $A$ are
  shaded.}
\label{fig:kenngr} 
\end{figure}



